Explainable Anomaly Detection: Counterfactual driven What-If Analysis

There exists three main areas of study inside of the field of predictive maintenance: anomaly detection, fault diagnosis, and remaining useful life prediction. Notably, anomaly detection alerts the stakeholder that an anomaly is occurring. This raises two fundamental questions: what is causing the fault and how can we fix it? Inside of the field of explainable artificial intelligence, counterfactual explanations can give that information in the form of what changes to make to put the data point into the opposing class, in this case "healthy". The suggestions are not always actionable which may raise the interest in asking "what if we do this instead?" In this work, we provide a proof of concept for utilizing counterfactual explanations as what-if analysis. We perform this on the PRONOSTIA dataset with a temporal convolutional network as the anomaly detector. Our method presents the counterfactuals in the form of a what-if analysis for this base problem to inspire future work for more complex systems and scenarios.

==> SECTIONS/ML4AD.tex <==
The first module, seen in Fig. \ref{fig:architecture}, is ML for anomaly detection. 
Many important decisions need to be made about the model and the dataset. 
We utilize the Temporal Convolutional Network (TCN) for anomaly detection, as justified in Section \ref{sec:background}. 
TCNs have shown to perform well on time series data similarly to Recurrent Neural Networks \cite{ribeiro2022online, Ferraro2023-jv}, Convolutional Neural Networks \cite{Solis-Martin2023-po, mey2022explainable, Grezmak2020-uu}, and Transformer-based architectures \cite{chen2022utrad, ma2021remaining}.
While these other architectures could make good choices, we chose our model as justified in Section \ref{sec:background}. 
As described in more detail in Section \ref{sec:experiment}, we utilize four different but similar TCN models for our training experiment as well as three models for our k-fold cross validation experiment. 

We perform our experiments on the PRONOSTIA\cite{nectoux2012pronostia} fault bearing dataset.
This dataset is chosen for its relative simplicity and notoriety as a PdM benchmark, so this dataset would serve as a good proof-of-concept. 
We also point to other datasets such as CMAPSS \cite{saxena2008turbofan} and XJTU-SY \cite{wang2018hybrid} as other potential benchmarks that both have equal validity as PdM benchmarks.
Additional information about the PRONOSTIA dataset can be seen in Section \ref{sec:experiment}.








%The machine learning element of our framework is open for much discussion. \hl{needs to be cleaned up} There are numerous datasets, such as the PRONOSTIA\cite{nectoux2012pronostia}, CMAPSS \cite{saxena2008turbofan}, XJTU-SY \cite{wang2018hybrid} and more, that would qualify for proper anomaly detection.  The only requirement required for the dataset would be a time-series dataset with at least two classifications, healthy and anomalous.  We utilize the Femto bearing dataset as a proof of concept for our framework, and thus, we describe the dataset below. Additionally, the black-box model serves as a general idea of an accurately performing model. Many different architectures show to perform well on time series data, such as Recurrent Neural Networks \cite{ribeiro2022online, Ferraro2023-jv}, Convolutional Neural Networks \cite{Solis-Martin2023-po, mey2022explainable, Grezmak2020-uu}, and Transformer-based architectures \cite{chen2022utrad, ma2021remaining}.While all of these models are subject to use, we utilize the Temporal Convolutional Network (TCN), as justified in Section \ref{sec:background}, which is described in more detail in Section \ref{sec:experiment}

==> SECTIONS/architecture_diagram.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{FIGURES/architecturev1.png}
    \caption{Data Flow Model of Counterfactuals for Anomaly Detection \hl{alter for two modules}}
    \label{fig:architecture}
\end{figure*}

==> SECTIONS/counterfactual_as_whatif.tex <==
\subsection{Counterfactuals as What-If Analysis}


==> SECTIONS/data.tex <==
\subsection{PRONOSTIA Bearing Dataset}
The PRONOSTIA bearing dataset was proposed in 2012 by Nectoux et al. \cite{nectoux2012pronostia} as a platform for bearing health assessment, diagnostics, and prognostics. 
This platform provides real data of bearing degradation under varying forces and speeds. 
This dataset in its totality consists of six training subsets and eleven testing subsets. 
The six training subsets consists of two per operational setting, known as ``Bearing1," ``Bearing2," and ``Bearing3." 
Additionally, the testing subsets consists of five for operational setting Bearing1, five for the operational setting Bearing2, and one for the last operational setting Bearing3. 
The dataset consists of rotational and temperature data. 
The rotational data consists of an acceleration value of the horizontal axis of the bearing and an acceleration values of the vertical axis of the bearing. 
The temperature data was not utilized for this experiment as it was not available for all of the different subsets. 

\subsection{Synthetic Minority Oversampling Technique (SMOTE)}
\cite{niaz2022class, Chawla2002-ub, Fernandez2018-ld}

==> SECTIONS/tcn.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{FIGURES/tcn.png}
    \caption{Temporal Convolutional Network Architecture}
    \label{fig:tcn}
\end{figure}

\subsubsection{Temporal Convolutional Network}


==> SECTIONS/usecase.tex <==
What-if analysis, as stated in Section \ref{sec:background}, is a method of simulating data to make decisions about the future. 
We apply this idea to PdM by utilizing ML for anomaly detection and counterfactual explanation generation as a method of simulating the data for our what-if analysis.
As seen in Fig. \ref{fig:architecture}, we utilize a framework made up of five main components: data and model selection, model training, model testing, space partitioning tree, and counterfactual generation. 
These five components can be abstracted into two modules: machine learning for anomaly detection and counterfactual generation. 
These modules are described in Section \ref{sec:ml4ad} and Section \ref{sec:comte}.
